Preprocessing Ambiguous Imprecise Points

Let ${R} = \{R_1, R_2, ..., R_n\}$ be a set of regions and let $ X = \{x_1, x_2, ..., x_n\}$ be an (unknown) point set with $x_i \in R_i$. Region $R_i$ represents the uncertainty region of $x_i$. We consider the following question: how fast can we establish order if we are allowed to preprocess the regions in $R$? The preprocessing model of uncertainty uses two consecutive phases: a preprocessing phase which has access only to ${R}$ followed by a reconstruction phase during which a desired structure on $X$ is computed. Recent results in this model parametrize the reconstruction time by the ply of ${R}$, which is the maximum overlap between the regions in ${R}$. We introduce the ambiguity $A({R})$ as a more fine-grained measure of the degree of overlap in ${R}$. We show how to preprocess a set of $d$-dimensional disks in $O(n \log n)$ time such that we can sort $X$ (if $d=1$) and reconstruct a quadtree on $X$ (if $d\geq 1$ but constant) in $O(A({R}))$ time. If $A({R})$ is sub-linear, then reporting the result dominates the running time of the reconstruction phase. However, we can still return a suitable data structure representing the result in $O(A({R}))$ time. In one dimension, ${R}$ is a set of intervals and the ambiguity is linked to interval entropy, which in turn relates to the well-studied problem of sorting under partial information. The number of comparisons necessary to find the linear order underlying a poset $P$ is lower-bounded by the graph entropy of $P$. We show that if $P$ is an interval order, then the ambiguity provides a constant-factor approximation of the graph entropy. This gives a lower bound of $\Omega(A({R}))$ in all dimensions for the reconstruction phase (sorting or any proximity structure), independent of any preprocessing; hence our result is tight.

==> oldLowerbound_29_11_18 <==
paragraph{Interval graph entropy.} 

Consider the problem of sorting a set of elements given a poset $P$ (not necessarily an interval order). It is well known that any poset can be represented as a directed graph $G(P)$. 
Khan and Kim \cite{kahn1995entropy} studied sorting posets and they discovered that $\log \T(P)$, the time it takes to sort an arbitrary poset $P$, is related to the entropy $H(P)$ of the graph  $G(P)$\footnote{There are various definitions of graph entropy and the one used in \cite{cardinal2013sorting} and \cite{kahn1995entropy} is based on the complement of  $G(P)$. 
See Appendix \ref{} for more details on graph entropy and previous results.}. Cardinal \etal \cite{cardinal2013sorting} improved the work of Khan and Kim and they gave an interesting geometric formula to compute the graph entropy if $P$ is an interval order.
In this paper, the poset which we want to sort is always an interval order induced from \RR. So from now on given $\RR$, we denote the entropy of a graph induced by the interval order by $H(\RR)$, and the number of linear extensions of this order by $\T(\RR)$.

Let $\RR$ be a set of (open) intervals in the combinatorial sense: for each interval $R_i$ we know which intervals intersect $R_i$, are contained in $R_i$, contain $R_i$ and are disjoint from $R_i$. Denote by $E(\RR)$ the infinite set of possible embeddings of $\RR$ between $(0,1)$. That is, each $E \in E(\RR)$ is a set of intervals where all the endpoints lie in $(0,1)$. Then Cardinal \etal prove:

\begin{lemma}[\cite{cardinal2013sorting}, Lemma 4  paraphrased]
\begin{equation}
    H(\RR) = \min_{E \in E(\RR)} \left\{ \frac{1}{n}  \sum_{R_i \in E}  -\log(|R_i|)   \right \}
\end{equation}
\end{lemma}

\begin{figure}[t]
\centering
\includegraphics[width =\linewidth]{entropy.pdf}
\captionsetup{width=\linewidth}
\caption{Let $\RR$ be a set of 5 intervals where 4 are disjoint and contained within a larger interval. We show 3 ways to embed these intervals between $[0, 1]$. The rightmost is the optimal one which shows that these intervals generate a poset with an entropy of around $0.5$.}
\label{fig:entropy}
\end{figure}

See Figure \ref{fig:entropy} for an extensive example. In the proof of Lemma 4, the authors note an interesting relation between $H(\RR)$ and $\log \T(\RR)$:

\begin{lemma}[Unnamed lemma in \cite{cardinal2013sorting}] 
\begin{align*}
   \log \T(\RR)  \le n \log n - n H(\RR)\le 2 \log \T(\RR) 
\end{align*}
\end{lemma}


We would like to use this information to relate the Ambiguity to $\log \T(\RR)$ however, the current definition of $H(\RR)$ makes algebraic reasoning in this setting awkward:
\begin{itemize}
    \item $H(\RR)$ lies in between $0$ and $\log n$ instead of $0$ and $n \log n$.
    \item The function $H(R)$ is smaller if the intervals $R_i$ are larger so the function somehow measures the opposite criterion.
    \item $n \log n = \sum_i \log n$. So this additional $n \log n$ intuitively scales the interior of $\log (|R_i|)$ by a factor n.
\end{itemize}


To combat these 3 issues we immediately introduce the following transformation: we measure the size of each interval in $\emph{units}$ of $\frac{1}{n}$. So if $n = 5$ and an interval $R_i$ has size $0.25$ we would say that the interval is $1.25$ units in size. In general we say that an interval $R_i$ in $[0,1]$ has size $S(R_i) = |R_i|*n$.
Note that $- \log(|R_i|) =  - \log( \frac{S(R_i)}{n}) = \log(n) - \log(S(R_i))$.
We perform a substitution to define a new function $F(\RR)$ which is algebraically more intuitive and we express the entropy $H(\RR)$ in terms of $F(\RR)$:

\begin{equation}
    F(\RR) := \max_{E \in E(\RR)} \left \{ \log \left( \prod_{R_i \in E}  S(R_i) \right) \right \}
\end{equation}

We can now rephrase the previous lemma in terms of $F(\RR)$:

\begin{lemma}
\begin{align*}
    F(\RR) \le 2 \log \T(\RR) 
\end{align*}
\end{lemma}
\begin{proof}

\begin{align*}
        n H(\RR) &=  n \cdot \min_{E \in E(\RR)} \left\{ \frac{1}{n}  \sum_{R_i \in E}  -\log(|R_i|)   \right \} \\
        &=  \min_{E \in E(\RR)} \left\{  \sum_{R_i \in E}  \log(n) - \log( S(R_i))   \right \} \\
        &=  n \log n - \max_{E \in E(\RR)} \left\{  \log \left(\prod_{R_i \in E}     S(R_i) \right) \right\}\\
    &= n \log n - \log (   F(\RR))
\end{align*}
\end{proof}


\paragraph{Ambiguity and Entropy} 

\begin{lemma}
\label{lemma:lowerbound}
Let $\pi$ be any containment-compatible permutation. Then: $\SO^\pi(\RR) \le  2 F(\RR)$
\end{lemma}

$S(R_i)$ is the length of an interval $R_i$ if we would not embed it on $(0,1)$ but on $(0,n)$.  $F(\RR)$ is the maximum over all embeddings in $(0, n)$ of the product of the lengths of the intervals in the embedding.  So to prove the inequality, we will create an embedding $E \in E(\RR)$ such that:

\[
\SO^\pi(\RR) = \log \left( \prod_{R_i \in \RR} |\Gamma_i| \right) \le \log \left( \prod_{R_i \in E} S(R_i)^2 \right) \le 2 F(\RR)
\]

We start with the original embedding of $\RR$ and we sort all the endpoints from left to right. To each endpoint $p$ (both left and right) we assign the coordinate $\frac{k}{2}$ if it is the $k$'th endpoint from left (indexing from 0). Observe that this is an embedding of $\RR$ on $(0,n - 0.5)$ where each interval $R_i$ has at least a size of $\frac{|\Gamma_i|}{2}$. This is because $\pi$ is a containment-compatible permutation, so each interval $R_i$ contains at least $\frac{|\Gamma_i|}{2} - 1$ endpoints on its domain.  Also note that between every rightmost endpoint and the next endpoint there is a distance of $\frac{1}{2}$. We translate every rightmost endpoint by $\frac{1}{2}$ to the right and create an embedding $E$ where each interval $R_i$ has size at least $\frac{|\Gamma_i|+1}{2}$. \\

Now let $A := \{ R_i \mid |\Gamma_i| = 1\}$, $B := \{ R_i \mid |\Gamma_i| = 2\}$, $C := \{ R_i \mid |\Gamma_i| = 3\}$ and $D := \RR \backslash \{A,B, C\}$. Let these sets contain $a, b, c$ and $d$ intervals respectively. Since each interval $R_i \in E$ has a size of at least $\frac{|\Gamma_i|+1}{2}$. We define $M$ as the product of the lengths of the intervals in $E$. Them we must have that:

\begin{equation}
\label{eq:base}
2^{F(\RR)} \ge M \ge 
    \left(\frac{2}{2}\right) ^a \left(\frac{3}{2}\right)^b   \left(\frac{4}{2}\right)^c \left(\frac{4}{2}\right)^d
\end{equation}


\begin{proof}[Proof of Lemma \ref{lemma:lowerbound}]

To prove the lemma we write $M$ in terms of the Ambiguity:
\[
2^{F(\RR)} \ge \prod_{R_i \in \RR}\! \frac{|\Gamma_i|+1}{2} 
\ge     \prod_{R_i \in A}\! |\Gamma_i| 
        \prod_{R_i \in B}\! \left( \frac{3}{4} \right) |\Gamma_i| 
        \prod_{R_i \in C}\! \left( \frac{2}{3} \right) |\Gamma_i|
        \prod_{R_i \in D}\! \left( \frac{1}{2} \right) |\Gamma_i|
    = \left( \frac{3}{4} \right)^b \left( \frac{2}{3}\right)^c \left( \frac{1}{2}\right)^d 2^{\SO^\pi(\RR)}\,.
\]
Then, using Equation~\ref{eq:base} we get 
\[
2^{F(\RR)}\cdot 2^{F(\RR)} \ge \left(\frac{3}{2}\right)^b   \left(\frac{4}{2}\right)^c \left(\frac{4}{2}\right)^d
\left( \frac{3}{4} \right)^b \left( \frac{2}{3}\right)^c \left( \frac{1}{2}\right)^d 2^{\SO^\pi(\RR)} \ge 2^{\SO^\pi(\RR)}\,,
\]
and therefore
\[
2F(\RR) \ge \SO^\pi(\RR)\,. \qedhere
\]
\end{proof}

This proves that the Ambiguity is also a lower-bound for the number of operations it takes to sort the values in $\RR$. We continue with showing that the Ambiguity is also (algebraically) an upper-bound with the following helper lemma:


\begin{lemma}
\label{lemma:helper}
Suppose $\RR$ can be partitioned into two disjoint sets $X$ and $Y$ where $X$ is to the left of $Y$. Then $F(\RR)$ is maximized if the intervals in $X$ together have width $|X|$ and if the intervals in $Y$ together have width $|Y|$.
\end{lemma}

\begin{proof}
Recall that  $2^{F(\RR)} := \max_{E \in E(\RR)} \left \{ \prod_{R_i \in E}  S(R_i) \right \}$ and that $S(R_i) := n|R_i|$ where $|R_i|$ is the "optimal" size for the region $R_i$ between $[0,1]$. This means that if the regions in $\RR$ are allowed to collectively have a width of $n$, that the optimal size of $R_i$ is some value $S(R_i)$. \\

We now define a new function $2^{F(\RR \mid x_1)} := \max_{E \in E(\RR)} \left \{ \prod_{R_i \in E}  S(R_i, x_1) \right \}$ where $S(R_i, x_1) = x_1|R_i|$. This function means that if the regions in $\RR$ are allowed to collectively have a width of $x_1$, that the optimal size of $R_i$ is some value $S(R_i, x_1)$. In particular:  $S(R_i, n) = S(R_i)$ which implies $2^{F(\RR \mid n)} = 2^{F(\RR)}$. 

\begin{align*}
    \forall x_1, x_2, \quad S(R_i, x_2) =  x_2 |R_i| = \left( \frac{x_2}{x_1}  \right) S(R_i, x_1). \\
    \textit{It follows that: } 2^{F(X \mid x_2)} =   \left( \frac{x_2}{x_1} \right)^{|X|} 2^{F(X \mid x_1)}
\end{align*}

If the intervals in $X$ can occupy a width of at most $x$, then it is always optimal to give the intervals in $Y$ a total width of $n-x$ (since we are maximizing the product of the lengths). It follows that: $2^{F(\RR)} = \max_{x_1 \in [0,n]} \{ 2^{F(X \mid x_1)} 2^{F(Y \mid n - x_1)} \}$. These two observations guarantee that $F(\RR)$ is maximal if $x_1 = |X|$ and this implies the lemma.
\end{proof}






\begin{lemma}
Let $\pi$ be any containment-compatible permutation. Then $F(\RR) \le 3 D^\pi(\RR)$
\end{lemma}

\begin{proof}
In Section \ref{sec:defs} we defined $\RR_{\le i}$ as the prefix of $\RR$. We prove the lemma with induction on $\RR_{\le i}$. 

For $i=1$ both values are 1, so the lemma holds. So we assume that the lemma holds for an arbitrary $i$ and we prove it for $i+1$.
\begin{equation*}
    \textit{Induction Hypothesis: }  2^{F(\RR_{\le i} \mid i)} \le \left( 2^{ D^\pi(\RR_{\le i})} \right)^3. 
\end{equation*}

For $i+1$ we must embed the intervals on $[0, i+1]$. We know the value of the righthand side: $\left( 2^{ D(\RR_{(i+1)\le})} \right)^3 = |\Gamma_{i+1}|^3  \cdot \left(2^{ D(\RR_{\le i})}\right)^3$. For the lefthand side we make a distinction between two cases: $|\Gamma_{i+1}| = 1$ or otherwise. 

In the first case $R_{i+1}$ is disjoint from the other intervals. Lemma \ref{lemma:helper} guarantees that $R_{i+1}$ gets a size of 1. The remaining intervals get embedded with a total width of $i$ which they already had in the previous iteration. So $2^{F(\RR_{(i+1)\le} \mid i+1)} = 1 * 2^{ F(\RR_{i} \mid i) }$ and because of the induction hypothesis $2^{ F(\RR_{(i+1)\le} \mid i+1)} \le \left(2^{ D(\RR_{(i+1)\le})} \right)^3$.

In the second case $|\Gamma_{i+1}|$ is at least 2. The other intervals used to be embedded with total width $i$ and now with a total width of $i+1$. So each of them expands with at most a factor $\frac{i+1}{i}$ which implies:

\begin{equation*}
    2^{ F(\RR_{(i+1)\le} \mid i+1 )} \le |R_{i+1}|  \left( \frac{i+1}{i} \right)^i 2^{ F(\RR_{\le i} \mid i)} \le |R_{i+1}| \cdot e \cdot 2^{ F(\RR_{\le i} \mid i)}
\end{equation*}
There are $i - \Gamma_{i+1}$ intervals disjoint from $R_{i+1}$ so Lemma \ref{lemma:helper} guarantees that $|R_{i+1}|$, so $|R_{i+1}| \cdot e \le |\Gamma_{i+1}|^3$ and we have proven the lemma.
\end{proof}

\begin{corollary}
The global Ambiguity $\SO(\RR)$ is a constant-approximation for the entropy $\log(\T(\RR))$.
\end{corollary}




